Auditing and Achieving Intersectional Fairness in Classification Problems

Machine learning algorithms are extensively used to make increasingly more consequential decisions about people, so achieving optimal predictive performance can no longer be the only focus. A particularly important consideration is fairness with respect to race, gender, or any other sensitive attribute. This paper studies intersectional fairness, where intersections of multiple sensitive attributes are considered. Prior research has mainly focused on fairness with respect to a single sensitive attribute, with intersectional fairness being comparatively less studied despite its critical importance for the safety of modern machine learning systems. We present a comprehensive framework for auditing and achieving intersectional fairness in classification problems: we define a suite of metrics to assess intersectional fairness in the data or model outputs by extending known single-attribute fairness metrics, and propose methods for robustly estimating them even when some intersectional subgroups are underrepresented. Furthermore, we develop post-processing techniques to mitigate any detected intersectional bias in a classification model. Our techniques do not rely on any assumptions regarding the underlying model and preserve predictive performance at a guaranteed level of fairness. Finally, we give guidance on a practical implementation, showing how the proposed methods perform on a real-world dataset.

==> sections/04_implementation.tex <==
%We now discuss practical implementation of post-processing techniques from Section
%\ref{sec:post_processing}. For a binary predictor, we showed in Proposition \ref{prop:linear_programming} that the RTDP can be obtained by solving a linear programming problem. To compute $\hat{FPR}$ and $\hat{FNR}$, one can use any of the techniques introduced in Section \ref{sec:metrics}: smoothed empirical estimation, bootstrap estimation, or Bayesian modelling.
%
%For a score predictor, computing an RTDP is more challenging. We first provide a way to evaluate the expected loss function for arbitrary values of $\tau_{s}$, $\tpp$ and $\tpn$. The expected loss function is given in Equation \ref{eq:loss_function} and, by applying the law of total probability, can be rewritten as:
%\begin{equation*}
% \sum_{s \in A} \mu_{s} \, \left[\tilde{FPR}_{s}(1-\mus) \, l(0,1) + \tilde{FNR}_{s} \, \mus \,  l(1,0)\right].
%\end{equation*}
%
%The unknown constant base rates $\mu_{s}$ and $\mus$  can be estimated from the data via any of the techniques from Section \ref{sec:metrics}. To compute the post-processed metrics $FNR^{\star}_{s}$ and $FPR^{\star}_{s}$ (cf. Definition \ref{def:post_metrics_no_randomization}), we first apply the thresholds to validation set's scores. We then estimate the metrics by using either bootstrap or Bayesian techniques as in Section \ref{sec:metrics}. The values of $\tilde{FNR}_{s}$ and $\tilde{FPR}_{s}$ can then be readily computed as:
%\begin{align*}
%\tilde{FPR}_{s} &= TNR^{\star}_{s} \, \tpn + FPR^{\star}_{s} \, \tpp, \\
%\tilde{FNR}_{s} &= FNR^{\star}_{s} \, (1-\tpn) + TPR^{\star}_{s} \, (1-\tpp).
%\end{align*}
%
%Since $FNR^{\star}_{s}$ and $FPR^{\star}_{s}$ are estimated directly from the data, they are piecewise constant functions of the threshold $\tau_{s}$. Therefore,  gradient-based optimization routines are unlikely to succeed as the gradient of the objective function -- if defined -- will be zero at all points. Moreover, the optimum will not be unique.
%
%To address this issue, we propose to smoothen the objective function by smoothing out model performance metrics. In particular, we construct random variables $\hat{Y}_{0,s} = (\hat{Y}|Y=0,S=s)$ and $\hat{Y}_{1,s} = (\hat{Y}|Y=1,S=s)$. We model them both as Beta random variables and estimate their parameters by maximum likelihood estimation.  We finally set $FPR^{\star}_{s}= 1-CDF_{\hat{Y}_{0,s}}(\tau_{s})$ and $FNR^{\star}_{s} = CDF_{\hat{Y}_{1,{s}}}(\tau_{s})$ for an arbitrary threshold $\tau_{s}$. This yields a smooth function that preserves monotonicity as depicted in Figure \ref{fig:fpr_smoothing}.  
%
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=\columnwidth]{img/fpr_smoothing.pdf}
%\Description{As a finite number of instances is available in the dataset, estimate of FPR are the same for different values of the threshold $\tau_{s}$. If no smoothing is applied, FPR is a step-wise function of the threshold. By using the proposed technique, FPR appears as a smooth monotonic curve.}
%\caption{Illustrative example of FPR for individuals with combination of sensitive attributes $s$ as a function of the threshold $\tau_{s}$.  Red points represent estimates of the FPR, the blue interpolating line depicts the non-differentiable step function, and the orange line is the smoothed curve obtained via a Beta modelling approach. }
%\label{fig:fpr_smoothing}
%\end{figure}
